What Matters for Ad-hoc Video Search? A Large-scale Evaluation on TRECVID

For quantifying progress in Ad-hoc Video Search (AVS), the annual TRECVID AVS task is an important international evaluation. Solutions submitted by the task participants vary in terms of their choices of cross-modal matching models, visual features and training data. As such, what one may conclude from the evaluation is at a high level that is insufficient to reveal the influence of the individual components. In order to bridge the gap between the current solution-level comparison and the desired component-wise comparison, we propose in this paper a large-scale and systematic evaluation on TRECVID. By selected combinations of state-of-the-art matching models, visual features and (pre-)training data, we construct a set of 25 different solutions and evaluate them on the TRECVID AVS tasks 2016--2020. The presented evaluation helps answer the key question of what matters for AVS. The resultant observations and learned lessons are also instructive for developing novel AVS solutions.

==> dataset-descrip.tex <==
\noindent\emph{The (Pre-)training datasets we used in the AVS task are as follow:}
\begin{itemize}
\setlength{\itemsep}{0pt}
\setlength{\parsep}{0pt}
\setlength{\parskip}{0pt}
    \item MSR-VTT~\cite{JunXu2016MSRVTT}: MSR-VTT is a common dataset in text-video retrieval tasks, which is a large-scale video description dataset. It contains 10K video clips with 41.2 hours and 200K clip-sentence pairs.
    % It collects 118 videos per query of 257 popular queries and filters manually to 7,180 videos. From the videos, it selects 10K video clips with 41.2 hours and 200K clip-sentence pairs.
    \item TGIF~\cite{tgif2015}: This dataset contains 100k animated GIFs (image sequences in general) from Tumblr and 120K natural language description from crowdsourcing. It collects 78,799 clips for training, 10,705 clips for validation, 11,351 clips for testing.
    \item VATEX~\cite{vatex2019}: This is a data set that describes human activities. It's a subset of the kinetics-600\cite{kinetics600} short-video collection,  Each video is associated with 10 sentences. It collects 23,896(25991) clips for training, 2,773(3000) clips for validation, 5570(6000) clips for testing. Since some data are not downloaded correctly, the VATEX dataset we use is not consistent with its original quantity.
    \item MSCOCO~\cite{mscoo2014}: MSCOCO is a large-scale image captioning dataset. It contains 123,287 images, and 5 manually annotated sentences per image.
    \item GCC~\cite{gcc2018}: Google's Conceptual Captions (GCC) consists of about 3,318,333 (image, sentence) pairs harvested from the web. The raw sentences are harvested from the Alt-text HTML attribute associated with web images. Finally, we successfully downloaded 1,925,125 pairs.
\end{itemize}
\noindent\emph{The validation datasets of AVS as follow:}
\begin{itemize}
\setlength{\itemsep}{0pt}
\setlength{\parsep}{0pt}
\setlength{\parskip}{0pt}
    \item TV16-VTT-train~\cite{awad2016trecvid}: The validation set is the training set of the TRECVID 2016 Video-to-text task. It contains 200 videos and 400 sentences. 
\end{itemize}
\noindent\emph{The testing datasets of AVS as follow:}
\begin{itemize}
\setlength{\itemsep}{0pt}
\setlength{\parsep}{0pt}
\setlength{\parskip}{0pt}
    \item IACC.3~\cite{awad2016trecvid}: Internet archives collection (IACC.3), the official test set for the TRECVID AVS in 2016–2018, contains 600 hours of video, 90 ad-hoc queries and available ground truth. 
    \item V3C1~\cite{V3C1Fabian2019}: Vimeo Creative Commons Collection (V3C1), the official test set for the TRECVID AVS in 2019–2021, contains 1000 hours of video. 70 ad-hoc queries and 50 of which available ground truth. 
    % This dataset includes 70 textual queries and 50 of which have published ground truth so far.
    % and is being used at the annual TRECVID international content-based video retrieval evaluation benchmark.
\end{itemize}


==> tab_abbreviate.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\normalsize
\renewcommand\arraystretch{1}
\centering

\begin{center}
\begin{tabular}{|l|l|}
\hline
\textbf{Abbreviate} & \textbf{Composition} \\ \hline
M & MSR-VTT \\ \hline
T & TGIF \\ \hline
V & VATEX \\ \hline
C & MS-COCO \\ \hline
G & GCC \\ \hline
M+T & Train on MSRVTT and TGIF \\ \hline
M+T+V & Train on MSRVTT, TGIF and VATEX \\ \hline
M+T+V-G & \begin{tabular}[c]{@{}l@{}}Pre-train on GCC and \\ train on MSRVTT, TGIF and VATEX\end{tabular} \\ \hline
M+T+V-C & \begin{tabular}[c]{@{}l@{}}Pre-train on MS-COCO and \\ train on MSRVTT, TGIF and VATEX\end{tabular} \\ \hline
\textit{rx101} & \textit{resnext-101} video feature \\ \hline
\textit{re152} & \textit{resnet-152} video feature \\ \hline
\textit{tf} & \textit{timesformer} video feature \\ \hline
\textit{c3d} & \textit{c3d} video feature \\ \hline
\textit{ircsn} & \textit{ircsn} video feature \\ \hline
\end{tabular}
\end{center}

\caption{\textbf{The left column represents the abbreviate name for the set of datasets or video feature from the right column.} }
\label{tab:abbreviate}

\end{table}

==> tab_query645-658.tex <==
\begin{table}[htbp!]
\begin{center}
\scalebox{0.75}{
\begin{tabular}{ll}
\\\hline
id  & Query\\\hline
645 & a person wearing a necklace      \\
657 & a woman with short hair indoors                                     \\
650 & one or more people drinking wine                      \\
648 & a man in blue jeans outdoors                       \\
655 & one or more persons standing in a body of water                            \\
658 & two or more people under a tree                      \\\hline
\end{tabular}}
\end{center}
\caption{\textbf{Queries of TRECVID 2020 }.}
\label{tab:datasets}
\end{table}

==> tab_tv18-20.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]

\begin{center}

\scalebox{0.6}{
\begin{tabular}{|c|l|l|l|}
\hline
\multicolumn{1}{|l|}{\textbf{Year}} & \textbf{Top-3 TRECVID} & \textbf{VideoFeature} & \textbf{Train dataset} \\ \hline
\multirow{3}{*}{2018} & Rank 1~\cite{li2018renmin} & resnext101,resnet152 & MSR-VTT+TGIF \\ \cline{2-4} 
 & Rank 2~\cite{huang2018informedia} & resnet152,faster\_r-cnn & \begin{tabular}[c]{@{}l@{}}YFCC+Image-Shuffle+UCF101+\\      Kinetics+Place+Google-Sports+\\      MSCOCO+Flickr30K+MSR-VTT\end{tabular} \\ \cline{2-4} 
 & Rank 3~\cite{bastan2018ntu} & resnet101,c3d,VGGish-network & MSRVTT+MSVD \\ \hline
\multirow{3}{*}{2019} & Rank 1~\cite{wu2019hybrid} & resnet152 & \begin{tabular}[c]{@{}l@{}}MSR-VTT+TGIF+IACC.3+\\      TRECVID2016-VTT\end{tabular} \\ \cline{2-4} 
 & Rank 2~\cite{li2019renmin} & resnext101,resnet152,c3d & MSR-VTT+TGIF+MSVD \\ \cline{2-4} 
 & Rank   3~\cite{ueki2019waseda_meisei_softbank} & resnet50,resnet101,resnet152 & \begin{tabular}[c]{@{}l@{}}Flickr8k+Flickr30k+MS-COCO+\\      GCC\end{tabular} \\ \hline
\multirow{3}{*}{2020} & Rank 1~\cite{zhao2020ruc_aim3} & resnext101,ircsn152 & MSR-VTT+TGIF+VATEX \\ \cline{2-4} 
 & Rank 2~\cite{lirenmin} & resnext101,resnet152,c3d & \begin{tabular}[c]{@{}l@{}}MSR-VTT+TGIF\\      (GCC for pre-training)\end{tabular} \\ \cline{2-4} 
 & Rank 3~\cite{wuvireo} & resnet152,faster\_r-cnn,P3D & \begin{tabular}[c]{@{}l@{}}MSR-VTT+TGIF+\\      VidOR-MPVC\end{tabular} \\ \hline
\end{tabular}
}
    
\end{center}

\caption{\textbf{Video feature and training dataset used by top 3 teams in TRECVID 2018-2020}}
% \label{tab:text encoder}
\end{table}

